Discovery of a Pulsar Wind Nebula Candidate Associated with the Galactic PeVatron 1LHAASO J0343+5254u

The astronomical origin of the most energetic galactic cosmic rays and gamma rays is still uncertain. X-ray followup of candidate "PeVatrons", systems producing cosmic rays with energies exceeding 1 PeV, can constrain their spatial origin, identify likely counterparts, and test particle emission models. Using 120 ks of XMM-Newton observations, we report the discovery of a candidate pulsar wind nebula, a possible counterpart for the LHAASO PeVatron J0343+5254u. This extended source has a power law X-ray spectrum with spectral index of 1.9 - softer at greater distance from the center - and asymmetric spatial extension out to 2'. We conduct leptonic modeling of the X-ray and gamma ray radiation from this complex system, showing that a fully leptonic model with elevated IR photon fields can explain the multiwavelength emission from this source, similar to other VHE pulsar wind nebulae; excess gamma ray emissivity not explained by a leptonic model may be due to hadronic interactions in nearby molecular cloud regions, which might also produce detectable astroparticle flux.

==> figures/spare_table.tex <==
\begin{deluxetable*}{lc|l|l}% C for mathmode
\tablecaption{MCMC best fit parameters and $2\sigma$ uncertainties for the leptonic and hadronic models} \label{tab:MCMCparam}
\tablewidth{\columnwidth}
\tablehead{ \colhead{Parameter} & \colhead{units} & \colhead{leptonic} & \colhead{hadronic}   }
\startdata
$E_{tot,p}$ & $\rm{erg}$ & & $(1.6 \pm 0.5) \times 10^{45}$ \\
$E_{tot,e}$ & $\rm{erg}$ & $(2.1 \pm 0.3) \times 10^{44}$  & \> \> $\rightarrow 1/3 \: E_{tot,p}$ \\
$E_{\rm{cut},p}$ & $\rm{TeV}$ & & $190 \pm 32$\\
$E_{\rm{cut},e}$ & $\rm{TeV}$ & $130 \pm 19$ & \> \> $\rightarrow 1/3 \: E_{\rm{cut},p}$ \\
$\alpha$ & & $2.0 \pm 0.2$ & $1.4 \pm 0.2$ \\
 & & & \\
$B$ & $\rm{\mu G}$ & $5.1 \pm 2.3$ & $2.1 \pm 0.7$ \\
$\kappa$ & & $61 \pm 15$ & \> \> $\rightarrow 1$ \\
$n_H$ & $\rm{cm^{-3}}$ & & $275 \pm 70$ \\
\enddata
\end{deluxetable*}
